CLLMs: Consistency Large Language Models

Parallel decoding methods such as Jacobi decoding show promise for more efficient LLM inference as it breaks the sequential nature of the LLM decoding process and transforms it into parallelizable computation. However, in practice, it achieves little speedup compared to traditional autoregressive (AR) decoding, primarily because Jacobi decoding seldom accurately predicts more than one token in a single fixed-point iteration step. To address this, we develop a new approach aimed at realizing fast convergence from any state to the fixed point on a Jacobi trajectory. This is accomplished by refining the target LLM to consistently predict the fixed point given any state as input. Extensive experiments demonstrate the effectiveness of our method, showing 2.4$\times$ to 3.4$\times$ improvements in generation speed while preserving generation quality across both domain-specific and open-domain benchmarks.

==> Consistency_LLM/figure_text/intro_observation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{Consistency_LLM/figures/intro_observation.pdf} 
\vskip -0.1in
\caption{An illustration demonstrates the ``fast-forwarded'' and ``stationary'' tokens in Jacobi decoding. Each point along the Jacobi trajectory is a color-coded sequence: blue for correct tokens matching with AR results, and red for inaccurate ones. Here, the token ``le'' is a stationary token that remains accurate despite the presence of preceding incorrect tokens. Two fast-forward tokens are ``0'' and ``cent'' at the $8$-th iteration step.
%This figure visualizes the prediction of $16$ tokens over $14$ Jacobi iterations, starting from a random point $0$ and ending at a fixed point $14$. 
}
\label{fig:intro_observation}
\vskip -0.1in
\end{figure}
